Incentivizing Reliable Demand Response with Customers' Uncertainties and Capacity Planning

One of the major issues with the integration of renewable energy sources into the power grid is the increased uncertainty and variability that they bring. If this uncertainty is not sufficiently addressed, it will limit the further penetration of renewables into the grid and even result in blackouts. Compared to energy storage, Demand Response (DR) has advantages to provide reserves to the load serving entities (LSEs) in a cost-effective and environmentally friendly way. DR programs work by changing customers' loads when the power grid experiences a contingency such as a mismatch between supply and demand. Uncertainties from both the customer-side and LSE-side make designing algorithms for DR a major challenge. This paper makes the following main contributions: (i) We propose DR control policies based on the optimal structures of the offline solution. (ii) A distributed algorithm is developed for implementing the control policies without efficiency loss. (iii) We further offer an enhanced policy design by allowing flexibilities into the commitment level. (iv) We perform real world trace based numerical simulations which demonstrate that the proposed algorithms can achieve near optimal social cost. Details can be found in our extended version.

==> S0-abstract.tex <==
Demand response (DR) is a cost-effective and environmentally friendly approach for mitigating the uncertainties in renewable energy integration by taking advantage of the flexibility of customers' demands. 
However, existing DR programs suffer from either low participation due to strict commitment requirements or not being reliable in voluntary programs.
In addition, the capacity planning for energy storage/reserves is traditionally done separately from the demand response program design, which incurs inefficiencies.
Moreover, customers often face high uncertainties in their costs in providing demand response, which is not well studied in literature.

This paper first models the problem of joint capacity planning and demand response program design by a stochastic optimization problem, which incorporates the uncertainties from renewable energy generation, customer power demands, as well as the customers' costs in providing DR.
We propose online DR control policies based on the optimal structures of the offline solution. %we propose two algorithms, prediction based policy and linear policy.
%In particular, the linear policy can be implemented in a 
A distributed algorithm is then developed for implementing the control policies without efficiency loss. We further offer enhanced policy design by allowing flexibilities into the commitment level. 
We perform real world trace based numerical simulations. Results demonstrate that the proposed algorithms can achieve near optimal social costs, and significant social cost savings compared to baseline methods. 

%the inflexibility of commitment levels.
%In particular, these programs can be split into two classes depending on whether customers are fully committed or fully voluntary to provide demand response. 
%Full commitment makes customers reluctant to participate, while the load serving entity (LSE) cannot rely on voluntary participation for reliability and dispatchability considerations. 

%This paper first highlights the inefficiency of existing DR programs in either extracting demand flexibilities from customers or helping the LSE to reduce the demand for energy storages/reserves that are costly and not environmental friendly.
%Motivated by this, we propose a generalized DR framework called Flexible Commitment Demand Response (FCDR) to allow for explicit choices of the level of commitment. 
%Then a distributed stochastic optimization framework is designed to achieve social optimum.


